Data-driven modelling of nonlinear dynamics by barycentric coordinates and memory

We present a numerical method to model dynamical systems from data. We use the recently introduced method Scalable Probabilistic Approximation (SPA) to project points from a Euclidean space to convex polytopes and represent these projected states of a system in new, lower-dimensional coordinates denoting their position in the polytope. We then introduce a specific nonlinear transformation to construct a model of the dynamics in the polytope and to transform back into the original state space. To overcome the potential loss of information from the projection to a lower-dimensional polytope, we use memory in the sense of the delay-embedding theorem of Takens. By construction, our method produces stable models. We illustrate the capacity of the method to reproduce even chaotic dynamics and attractors with multiple connected components on various examples.

==> Notation.tex <==


Notation...

$x_t$ is a data vector at time $t$
$\Xi$ is matrix... 


$\sigma_k$ are vectors... 
$\Sigma$  is also a matrix,

$\gamma_t$ is vector in time
$\Gamma$ is also matrix...

$\Lambda$ is a matrix...

$f$ for generator.
$g$ is the observable...

Random Variables (need notation)
Path Probabilities (needs notation $p( X = x )$)


Memory Operator (\psi)

Error Functions (need notation)

Indices...

dimension 'D' , d is the index

time 'T' , t is index 

vertex 'K' , k in index

memory 'M', m in index

Subscript and superscript ...

Time subscript
vertex superscript
memory subscript $(\hat{\Lambda}_M)$










==> SPA.tex <==
\section{Scalable Probabilistic Approximation (SPA)}
\label{sec:spa}

Data driven methods for learning dynamics entail two fundamental steps: the first being \emph{feature selection} and the second being \emph{dynamics reconstruction}. 
The first step entails projecting the data into a known \emph{feature space} to help delineate the underlying dynamics of the data.
Then, in the second step, a \emph{propagator} over the projected data in the feature space is inferred which recapitulates the dynamics of the original data.
The choice in feature spaces is a key bottleneck for most datasets. This is particularly so for high-dimensional datasets, where feature spaces which capture the right geometry of the data, in practise, are found to be sensitive to noise and ill-conditioned when inferring the propagator. 
One method which balances the choice of an interpretable feature space and the stability of the propagator is the \emph{Scalable Probabilistic Approximation} (SPA) method~\cite{spaPaper,eSPAIllia}.


Like other data driven methods, the principle behind SPA is divided into two steps: the first to project the data onto a convex polytope and secondly to infer a linear propagator over the said polytope.
The first of the two steps, which we refer to as ``SPA I", is formulated as follows: for a sequence of $\timeT \in \N$ observations of $\dimD \in \N$ dimensional data points, $\data := [\datapoint_1\vert \cdots\vert\datapoint_\timeT],$ the $\clus \in \N$ vertex convex polytope to project the data onto is determined by solving for the matrices $\Smatrix \in \R^{\dimD \times \clus}$ and $\Gamma \in \R^{\clus \times \timeT}$ which satisfy:
\begin{equation*}
\tag{SPA I}
\begin{split}
&\hspace{2cm}[\Smatrix,\Gamma] = \argmin_{\Smatrix^*,\Gamma^*} \Vert \data - \Smatrix^*\Gamma^* \Vert_F,\\
\text{subject to,}& \\
& \Smatrix := [\Spoint_1\vert \cdots \vert \Spoint_K] \in \R^{\dimD\times K}, \quad \Gamma := [\gamma_1\vert \cdots\vert \gamma_\timeT] \in \R^{\clus\times \timeT},  \\
\text{with}&  \\
&\sum\limits_{k=1}^\clus \gamma_{t}^k = 1 \text{ and }  \gamma_{t}^k \geq 0 \text{ for all } t \in \{1,\ldots, T\}\text{ and }k \in \{1,\ldots, K\}. \\
\end{split}
\label{eq:SPA1}
\end{equation*}

We can deduce from the above formulation that $\sigma_\bullet,$ the columns of the matrix $\Smatrix,$ represent a new coordinates system consisting of $\clus$ basis in $\R^\dimD.$ Furthermore, $\gamma_\bullet,$ the column vectors of $\Gamma,$ are simply an orthogonal projection of data points $x_\bullet$ onto the convex polytope formed by the span of $\{\Spoint_1, \ldots , \Spoint_K \}.$ For each vertex $k \in \{1,\ldots, \clus \}$, the value of $\gamma_{\bullet}^k$ can be interpreted as a closeness/affiliation measure of the data point $\datapoint_\bullet$ to the vertex $\Spoint_k$. For brevity, here on in, we will refer to the ``convex polytope" spanned by vectors $\sigma_\bullet$ as simply a ``polytope" and denote it by $\mathcal{M}_\Smatrix.$ Further, we call a vector $\gamma$ that describes the position of a point $\datapoint$ in $\mathcal{M}_{\Sigma}$ the \textit{barycentric coordinate} of $\datapoint$ with respect to $\Sigma$.

\iffalse

\begin{example}

Let us consider the following 5-dimensional Lorenz-96-system, a coordinate-wise hierarchical continuous-time dynamical system, which is described by, 
\begin{equation*}
    \dot{x}^{(k)} = (x^{(k+1)} - x^{(k-2)})x^{(k-1)} - x^{(k)} + F \quad \text{ for } k = 1,\dots 5,
\end{equation*}
with initial condition $\datapoint_0 = (3.8,3.8,3.8,3.8,3.8001)$ and $F = 3.8.$ Higher values of the parameter $F$ cause the system to become chaotic, we choice our $F$ to generate a fairly non-chaotic behaviour. Evolving this system forward, after the transient phase, we saw that the system exhibits a periodic behaviour in all dimensions (Figure~\ref{fig:Lorenz96_introductionPlot} a.). Looking at the trajectory of the system two dimensions at a time reveals that the trajectory of the system does look on it elf in time and also has a sharp directional change (Figure~\ref{fig:Lorenz96_introductionPlot} a. black arrows). Then, a  \eqref{eq:SPA1} projection of  the trajectory onto a polytope with three vertices (face of a triangle), showed that the trajectory on the polytope forms a trace of two overlapping rings (Figure~\ref{fig:Lorenz96_introductionPlot} b.). Both rings were surprisingly the same size, in contrast, in the original trajectory, we saw that the two loops on either side of the overlap point have vastly different radii. Furthermore, we saw that the trajectory on the polytope touches all three edges of the polytope, indicating that some geometric information (such as derivatives) are lost for these points after projecting into the polytope (Figure~\ref{fig:Lorenz96_introductionPlot} b. black arrows). Lastly, looking into the projection error of \eqref{eq:SPA1} compared to \emph{Principle Component Analysis} (PCA)~\cite{jolliffe} for increasing number of vertices, we found that the projected error between $K$-vertices and $K$-principle components was very similar (Figure~\ref{fig:Lorenz96_introductionPlot} c.). This tells us that the compression capacity of projecting into the polytope is comparable to PCA.  

%We generate a trajectory of length $16$ with a step size of $0.01$, in consequence creating $1601$ data points. As initial value we chose $\datapoint_0 = [3.8,3.8,3.8,3.8,3.8001]^T$. We truncate the first $600$ time steps to give it time to converge towards the attractor of the system, leaving us with $1001$ data points.

\begin{figure}[ht!]
\centering
\includegraphics[width=\textwidth]{Bilder/Example_1_Fig.pdf}
\caption{(a) All pairs of coordinates of the Lorenz 96 system with $F = 3.8$. (b) Coordinates of $\gamma_t$ from the SPA I computation with $K = 3$. (c) Average relative Euclidean reconstruction error per data point with varying values for $K$ and with PCA.}
\label{fig:Lorenz96_introductionPlot}
\end{figure}
\label{example:Lorentz96}
\end{example}

\fi

\begin{remark}
The idea of projecting on a convex polytope derived from the data has emerged in different sciences under different names, e.g. Archetypal Analysis~\cite{cutler} in computer science and PCCA+~\cite{weberpcca} in chemistry. The key motivation being that the vertex have clear interpretabiltiy given they are points in the data-space. \nw{Are the grammatics correct? I don't quite understand the sentence.} Furthermore, all points projected into the polytope have no projection error. \nw{Do you mean points that are inside the polytope?} However, on the downside it is linear decomposition of the data, meaning, nonlinear trajectories in the data-space will still be nonlinear on the polytope. 

The key motivation is that the vertices have clear interpretability given they are points in the data-space. Furthermore, all points that lie inside the polytope have no projection error. \nw{Do you mean points that are inside the polytope?} However, on the downside it is a linear decomposition of the data, meaning, nonlinear trajectories in the data-space will still be nonlinear on the polytope. 
\end{remark}


After embedding the data points from $\R^\dimD$ into $\mathcal{M}_\Sigma,$ the second step of SPA is to find a column-stochastic matrix $\Lambda \in \R^{\clus \times \clus} $ which propagates the projected points in the polytope. We refer to this step as ``SPA II", and formulate it as follows: let the matrices $\Smatrix \in \R^{\dimD \times \clus}$ and $\Gamma \in \R^{\clus \times \timeT}$ be the solution to \eqref{eq:SPA1} for a dataset $\data := [\datapoint_1\vert \cdots\vert\datapoint_\timeT],$ then find $\Lambda$ such that,
\begin{equation*}
\tag{SPA II}
\begin{split}
\Lambda &= \argmin_{\Lambda^*} \Vert [\gamma_2 \vert \cdots \vert\gamma_\timeT] - \Lambda^* [\gamma_1 \vert \cdots\vert\gamma_{\timeT-1}] \Vert_F, \\
\text{satisfying,} & \\
& \Lambda \succeq 0 \text{ and } \sum_{k=1}^K \Lambda_{k,\bullet} = 1. 
\end{split}
\label{eq:SPA2}
\end{equation*}
The propagator $\Lambda$ gives a relation that describes the evolution of the original system on the polytope $\mathcal{M}_\Sigma.$ Furthermore, $\Lambda$ being a column-stochastic matrix guarantees that the image of $\mathcal{M}_{\Sigma}$ is again inside the polytope $\mathcal{M}_{\Sigma}$. In practice, the properties of the \eqref{eq:SPA2} propagator is more stable and well-conditioned compared to other data-driven methods. Another advantage of the SPA method is that the matrix $\Sigma: \mathcal{M}_\Sigma \rightarrow \R^\dimD$ gives a natural lifting of the polytope back into the full data-space $\R^\dimD.$ For example, for two data points $x_t$  and $x_{t-1},$ we can estimate $x_t$  by, $ \datapoint_{t} \approx \Smatrix\, \gamma_{t} = \Smatrix \Lambda\, \gamma_{t-1},$ where we first project $x_{t-1}$ to  $\gamma_{t-1}$ in the polytope $\mathcal{M}_\Sigma$, then propagate it forward using $\Lambda,$ and then lift it back into $\R^\dimD$ using $\Sigma.$

Though the full system might be nonlinear, using the SPA method reduces the learning of the dynamics on the data-space to learning a linear system on a convex polytope. To date, the literature on the translation of the dynamics after projecting into a polytope is sadly vacuous. For this reason, we will briefly formalise and give commentary on the SPA method in the context of dynamical systems in the following section, but first, we will build further intuition for \eqref{eq:SPA2} by studying its application on the Lorenz 96 from Example~\ref{example:Lorentz96}.
\begin{example}[Example~\ref{example:Lorentz96} continued: SPA II predictions on the Lorenz 96 system]
For $K = 3,\dots,6$, we used the resulting $\Lambda$ from \eqref{eq:SPA2} to make one-step predictions. The dynamics of $\gamma_t$ became more complex with increasing $K$, since more of the true trajectory of the $\datapoint_t$ in $\R^5$ was captured.  Out of the trajectory of $1000$ time steps of length $0.01$, we used the first $600$ time steps for training in SPA II and the remaining $400$ for testing. For the predictions, we used different step sizes, resulting in different models for each. Making a prediction with a time step of length $\Delta t$ then meant mapping $\gamma_t$ to $\gamma_{t+ \Delta t}$. 

As Figure~\ref{fig:Lorenz96_ExampleSPAII_onestep} shows, with higher step sizes, the predictions of the linear model generated by $\Lambda$ were circles with decreasing radii. The prediction errors thus increased with the step size. As error measure, we computed the average Euclidean error between prediction and true data point, resp. $\gamma_t$ over all time steps (defined as the average one-step \tgammaerror in Appendix \ref{sec:App_errors}). The errors in $\gamma_t$ were comparable between the different $K$ for small time steps, possibly because the dynamics in $\gamma_t$ are simpler with small $K$. After lifting up into the true data space, we derived an acceptable error (the average \ttruespaceerror defined in Appendix \ref{sec:App_errors}) only with $K = 5$ and $K = 6$, since the lifting of the $\gamma_t$ could only lie on a $K-1$-dimensional manifold, so that the prediction error was lower-bounded by the projection loss depicted in Figure~\ref{fig:Lorenz96_introductionPlot}. Note that, before performing SPA 1 and SPA II, we had normalized the data to the cube $[-1,1]^5$ by a linear shifting and scaling.
\begin{figure}[ht!]
\centering
%\includegraphics[width=\textwidth]{Bilder/Lorenz96_ExampleSPAII_onestep.png}
%\includegraphics[width=\textwidth]{Bilder/Lorenz96_SPA2_predictions.png}
\includegraphics[width=\textwidth]{Bilder/SPAII_onestep_Fig3_all.png}
\caption{Top and middle row: first two coordinates of one-step \ref{eq:SPA2} predictions in $\gamma_t$ with $K = 3$ for different step sizes. Bottom row: average one-step Barycentric coordinate and true space error prediction error for $K = 3,\dots,6$.}
\label{fig:Lorenz96_ExampleSPAII_onestep}
\end{figure}
\end{example}
\FloatBarrier


\begin{remark}
Please note that in the original SPA paper~\cite{spaPaper}, the authors refer to \eqref{eq:SPA1} as the SPA problem and refer to other literature for solving \eqref{eq:SPA2}. Hence, the notation of denoting the two problems by \eqref{eq:SPA1} and \eqref{eq:SPA2} comes from us. Further, in \cite{spaPaper}, the authors perform both the \ref{eq:SPA1} and \ref{eq:SPA2} steps together in one augmented step with the constraint that $\Lambda$ need to be an identity (Theorem~2 in \cite{spaPaper}). The authors prove that the solution to their one step approach is equivalent to the two step. Hence, the two approaches only differ in computing and not in mathematics. 
\end{remark}


\subsection*{SPA in the context of dynamical systems I}
\label{sec:SPAdynSystems}
In this section we explore formalism of modelling a dynamical system using SPA and its consequences. We begin by defining the map from the data space into the polytope.

%We need to formally introduce the projection into the polytope.


\begin{definition}
For $x \in \mathcal{M}$ and $\gamma$ a $K$ dimensional barycentric coordinate, we define the mapping of $x$ into a $K$-vertexed polytope characterised by $\Sigma$ as follows:

\textbf{Case 1: } for $K \leq D$:

\begin{equation}
\begin{split}
    &\hspace{1.6cm}\rho_\Sigma(\datapoint) := \argmin\limits_{\gamma^*}\Vert \datapoint - \Smatrix\gamma^*\Vert_2, \hspace{1cm} \text{s.t. } \gamma^*_\bullet \geq 0, \quad \Vert \gamma^* \Vert_1 = 1.
    \end{split}
    \label{eq:rhoK<D}
\end{equation}

\textbf{Case 2: } for $K > D$ : 
\begin{equation}
\begin{split}
    &\hspace{1.4cm}\rho_\Sigma(\datapoint,\gamma) := \argmin\limits_{\gamma^*} \Vert \gamma - \gamma^* \Vert_2 \\ & 
    \text{ s.t. }\gamma^* = \argmin\limits_{\gamma'}\Vert \datapoint - \Smatrix\gamma'\Vert_2
    \text{ with } \gamma_\bullet,\gamma^*_\bullet  \geq 0 \text{ and } \Vert \gamma \Vert_1, \Vert \gamma^* \Vert_1 = 1.
    \end{split}
    \label{eq:rhoK>D}
\end{equation}
\end{definition}

Case 2, $K > D,$ is interesting because there is no well-defined function that maps $\datapoint$s to $\gamma$s. For this reason, we define a function $\rho_\Sigma$ to be dependent not only on $\datapoint$ but also a reference $\gamma.$ This means that $\gamma_t = \rho_\Sigma(\datapoint_t,\gamma_{t-1})$ minimizes the distance between $\datapoint_t$ and $\Smatrix\gamma_t$ while $\gamma$ has to be closest to $\gamma_{t-1}$ among all those minimizers. This now makes the mapping into the polytope well defined. For Case 1, $K \leq D,$ we can always assume that the polytope is a $K-1$-dimensional simplex, furthermore, the map $\rho$ is also an orthogonal projection (see Appendix \ref{sec:App_rhosigma}).





\iffalse
In congruence with \eqref{eq:SPA1}, let $\Sigma$ be the matrix containing the $\clus$ vertices and $\mathcal{M}_\Sigma$ the polytope. We represent a point $\datapoint_t \in \R^\dimD$ (approximately) by \textit{barycentric coordinates} $\gamma_t \in [0,1]^K$. At this point, we need to distinguish two cases:

\textbf{Case 1: } $K > \dimD$: In this case, \eqref{eq:SPA1} can be solved exactly. Then although we can recover $\datapoint_t$ from $\gamma_t$ by multiplication with $\Smatrix$, the representation of $\datapoint_t$ in the basis of $\Smatrix$ need not be unique. As a consequence, there is no well-defined function that maps $\datapoint_t$ to $\gamma_t$. For this reason, we define a function $\rho_\Sigma$ that is dependent not only on $\datapoint_t$, but also on $\gamma_{t-1}$ by defining it as,

This means that $\gamma_t = \rho_\Sigma(\datapoint_t,\gamma_{t-1})$ minimizes the distance between $\datapoint_t$ and $\Smatrix\gamma_t$ while $\gamma$ has to be closest to $\gamma_{t-1}$ among all those minimizers. In this definition we assume that the minimizer of the distance to $\gamma_{t-1}$ among minimizers of $\Vert \datapoint_t - \Sigma \gamma \Vert_2$ is unique\footnote[2]{From a numerical point of view, we realize this by solving $\gamma_t = \argmin\limits_{\gamma_t} \Vert \datapoint_t - \Smatrix\gamma_t \Vert_2$ with the initial value of the numerical minimization problem given by $\gamma_{t-1}$. In this way, the numerical solver should always give a local minimizer of $\Vert \datapoint_t - \Smatrix\gamma_t \Vert_2$ that is close to $\gamma_{t-1}$.}.
\textbf{Case 2: } $K \leq \dimD$. Note that in the case $K \leq D$, $\mathcal{M}_{\Sigma}$ can be assumed to be a simplex.

\begin{lemma}
Let $\Sigma = [\sigma_1,\dots,\sigma_D] \in \R^{\dimD \times K}$ denote the vertices of a non-simplex polytope $\mathcal{M}_{\Sigma}$. Then there exists a simplex with vertices $\tilde{\Sigma}$ so that for points $[\datapoint_1\vert\cdots\vert\datapoint_T] \in \R^{\dimD}$, there exist barycentric coordinates $[\gamma_1\vert\cdots\vert\gamma_T] \in \R^K$ so that $\Vert [\datapoint_{1} \vert \cdots \vert\datapoint_\timeT] - \tilde{\Sigma} [\gamma_1\vert\cdots\vert\gamma_T] \Vert_F \leq \Vert [\datapoint_{1} \vert \cdots \vert\datapoint_\timeT] - \Sigma [\gamma_1\vert\cdots\vert\gamma_T] \Vert_F$.
\label{pro:rhosimplex}
\end{lemma}
\begin{proof}
For the proof, we simply observe that every polytope $\mathcal{M}_{\Sigma}$ with $K$ vertices that is not a simplex is at most $(K-2)$-dimensional. We can then use $K-1$ vertices to construct a simplex which contains $\mathcal{M}_{\Sigma}$ which already proofs the proposition. Since $K\leq \dimD$, we are then left with one vertex we can use to increase the dimension of the polytope by constructing a $(K-1)$-dimensional simplex.
\end{proof}
For example, assume $K = 4$ and $\dimD \geq 4$. Then if $\mathcal{M}_{\Sigma}$ were not a ($3$-dimensional) simplex, it would at most be 2-dimensional, given by a polygon with $4$ vertices. However, for such a polygon, we could construct a triangle which contains this polygon while we could use the fourth vertex to reduce the projection error by increasing the polytope to a third dimension. As a consequence, solutions of $\eqref{eq:SPA1}$ will typically form a $(K-1)$-dimensional simplex (if not, one could add a constraint to \eqref{eq:SPA1}). We therefore always assume $\mathcal{M}_{\Sigma}$ to be a simplex whenever $K \leq D$.

This allows us to proof the following Proposition.
\begin{proposition}
Let $\Sigma \in \R^{\dimD \times K}$. The function $\rho_\Sigma:\R^\dimD \rightarrow [0,1]^K$ defined as
\begin{equation}
    \rho_\Sigma(\datapoint) = \argmin_{\gamma} \Vert \datapoint - \Sigma \gamma \Vert_2 \quad \text{s.t. } \gamma_\bullet \geq 0, \quad \sum_{i=1}^K \gamma_i = 1
    \label{eq:rhoK<D}
\end{equation}
is well-defined for all $\datapoint \in \R^{\dimD}$.
\label{lem:rhowelldefined}
\end{proposition}
\begin{proof}
By denifition, the term $\Sigma \rho_\Sigma(\datapoint)$  is the closest point to $\datapoint$ in $\mathcal{M}_{\Sigma}$, so that it is the orthogonal projection of $\datapoint$ onto $\mathcal{M}_{\Sigma}$. This is always well-defined in Euclidean space. The question now is whether there exists $\tilde{\gamma}$ so that $\Sigma \gamma = \Sigma \tilde{\gamma}$. Since $\mathcal{M}_{\Sigma}$ is a simplex, the barycentric coordinates of the projection of $\datapoint$ onto $\mathcal{M}_{\Sigma}$ are unique~\cite{guessab}.
\end{proof}

Note that $\rho_\Sigma$ can be seen as an orthogonal projection of points in $\R^\dimD$ onto a $K$-vertexed simplex. The definition of $\rho_\Sigma$ in Eq.~\eqref{eq:rhoK<D} for the case $K \leq \dimD$ is equivalent with the one in Eq.~\eqref{eq:rhoK>D}, since the set of minimizers of $\Vert \datapoint - \Sigma \gamma \Vert_2$ contains only one element. We could equivalently write it as $\rho_\Sigma(\datapoint,\bullet)$ and use the definition from Eq.~\eqref{eq:rhoK>D}.
\fi

\iffalse
From a numerical point of view, we realize this by solving $\eqref{eq:SPA1}$ first to find suitable $\Spoint_i$ whose convex hull contains all data points, then solve
\begin{equation*}
    \gamma_0 = \argmin\limits_{\gamma} \Vert \datapoint_0 - \Smatrix\gamma \Vert_2
\end{equation*}
with a randomly chosen initial condition in the minimization algorithm which is a Spectral Projected Gradient method~\cite{birgin}. From then on, we iteratively solve
\begin{equation}
    \gamma_t = \argmin\limits_{\gamma_t} \Vert \datapoint_t - \Smatrix\gamma_t \Vert_2
    \label{eq:GammaSubproblem}
\end{equation}
with the initial value of the numerical minimization problem given by $\gamma_{t-1}$. In this way, the numerical solver should always give the minimizer of \eqref{eq:GammaSubproblem} that is closest to $\gamma_{t-1}$.
\fi

Let us consider a discrete dynamical system on a compact manifold $\mathcal{M}$ of the form,
\begin{equation*}
   \datapoint_t = \gener(\datapoint_{t-1}),
\end{equation*}
where $x_\bullet \in \mathcal{M}$ and $f:\mathcal{M} \rightarrow \mathcal{M}.$
For now, we restrict ourselves to the case $K > \dimD$. The opposite case will be discussed at the end of the next Section.

We obtain the following dynamical system for the $\gamma_{t}$:
\begin{equation}
    \gamma_t = \rho_\Sigma(\datapoint_t,\gamma_{t-1}) = \rho_\Sigma(\gener(\datapoint_{t-1}),\gamma_{t-1}) = \rho_\Sigma(\gener(\Smatrix\gamma_{t-1}),\gamma_{t-1}) =: \textbf{v}(\gamma_{t-1}).
    \label{eq:gammaDynSys}
\end{equation}
The function $\textbf{v}: \mathcal{M}_\Sigma \rightarrow \mathcal{M}_\Sigma$ now defines the dynamical system dependent on the $\gamma_\bullet$. Note that we denote by $\mathcal{M}_{\Sigma}$ both the polytope in $\R^\dimD$ and the simplex which contains the entries of $\gamma$. Both are connected by a smooth coordinate change given by multiplication with $\Sigma$, resp. its pseudo-inverse $\Sigma^+$. 

Hence, in \eqref{eq:SPA2}, we essentially approximate the function $\textbf{v} $ by a linear mapping given by the matrix $\Lambda$, that is, $\gamma_{t} \approx \Lambda \gamma_{t-1}.$ Furthermore, the long-term behaviour is thus approximated by
\begin{equation}
    \gamma_{t+i} = \textbf{v}^{i} (\gamma_{t}) \approx \Lambda^{i} \gamma_{t}.
    \label{eq:SPAII_dynamicsApproximation}
\end{equation}
The propagator $\Lambda$ being a column-stochastic matrix is good for keeping the predictions inside the polytope. However, $\Lambda$ is still only a linearisation of $\textbf{v},$ making it imprecise when $\textbf{v}$ is nonlinear (see also Appendix \ref{sec:App_SPAfixedpoints}). 

\begin{example}
\label{exa:Lorenz_Part3}
In this example, we investigated the ability of \ref{eq:SPA2} to make long-term predictions, again on the Lorenz-96-system.

By construction, $\Lambda$ is a column-stochastic matrix. As such, without additional constraints on the \eqref{eq:SPA2} problem, the dynamics induced by $\Lambda$ in Eq.~\eqref{eq:SPAII_dynamicsApproximation} will typically converge to a fixed point (see Appendix \ref{sec:App_SPAfixedpoints}). Therefore, non-linear dynamics cannot be well reconstructed over longer time spans. A commonly used method for the identification of nonlinear dynamics is Sparse Identification of Nonlinear Dynamics (SINDy~\cite{sindy,sindyc}), which in essence solves a nonlinear regression problem from $\datapoint_t$ to $\datapoint_{t+1}$ or, if available, $\dot{\datapoint}_t$. For this aim, the dynamics are projected into the span of basis functions.

For comparison, we used both \ref{eq:SPA2} and SINDy to make long-term forecasts and compare their prediction errors. As basis functions in SINDy, we chose all monomials up to degree $3$ and $\sin(k\datapoint), \cos(k\datapoint)$ for $k = 1,\dots,10$.

As we could see in Figure~\ref{fig:Lorenz96_Example_forecasting}, with a time step of $\Delta t = 0.08$, both methods were insufficient to reconstruct the dynamics well. While the model induced by SINDy made for a small error for the first $\sim 30$ steps but diverged then, the SPA II models generated trajectories that converged to a fixed point, as expected.
\begin{figure}[ht!]
\centering
%\includegraphics[width=\textwidth]{Bilder/Lorenz96_Example_forecasting.png}
\includegraphics[width=\textwidth]{Bilder/Lorenz96_SPAII_Fig4_all.png}
\caption{\textbf{a.}, \textbf{b.} and \textbf{c.} forecasts of $50$ steps with a step size of $0.08$ with the SPA II models identified with $K = 3$ and $K = 5$ and SINDy. SINDy manages to capture the behaviour for several steps but then diverges. The SPA II models both converge to a fixed point. \textbf{d.} average Euclidean forecast error with SPA II for $K=3,\dots,6$ and SINDy. In the long-term, all \ref{eq:SPA2} models are insufficient. SINDy generates a model that is accurate for several time steps but then diverges.}
\label{fig:Lorenz96_Example_forecasting}
\end{figure}
\end{example}

As Example \ref{exa:Lorenz_Part3} illustrates, the linear models generated with SPA II were generally insufficient for longer-term forecasting of nonlinear dynamics. But system identification methods that are based on basis functions carry the danger of divergence. Plus, one has to choose appropriate basis functions.

Especially for high-dimensional systems, these issues can make typical approaches for system identification infeasible and yield the need for application of a dimension reduction technique first. However, if the data do not lie inside a low-dimensional polytope, then, as we have seen, one has to live with a high projection loss, which is also the case in SPA. Moreover, we cannot formulate the dynamics of the $\gamma_t$ as done in Eq.~\eqref{eq:gammaDynSys} since there does not exist a surjective mapping from $\gamma_t$ to $\datapoint_t$. In Section~\ref{sec:memory}, we will introduce a method that takes the projection error into account and propagates states inside the polytope in a nonlinear way. In this way, we will be able to leverage the benefit of, e.g., SINDy in identifying nonlinear dynamics while doing this in a feasible dimension and keeping the dynamics inside the bounded domain formed by the polytope. At the end, we will illustrate how to lift the projected dynamics back up the the full data space.



%We now use the propagator computed in \eqref{eq:SPA2} to predict states of the system. For this, we use different values of $K$ and different step sizes with which we fit the model. We always predict a time of $0.32$ ahead, but with different step sizes, given by $0.01,0.02,0.04,0.08,0.16,0.32$. As a consequence, we have to take $32,16,\dots,1$ steps with the model. We compute the average error for a forecast of $0.32$ and show the result in Fig. \ref{fig:Lorenz96_errorPlot_overK}.
%As we can see, an increase of $K$ generally increases the prediction quality. As a comparison, we show the error generated with SINDy with basis functions chosen as all monomials up to degree $2$.

%As is natural with SINDy, higher step sizes yield higher predictions errors while with a small step size can capture the dynamics of the system so that the prediction quality is good even if several (i.e., $16$ or $32$) steps are taken. With SPA, the opposite is the case. This might seem counter-intuitive but can easily be explained: as a linear model, trajectories created with it will converge to a fixed point in most cases and thus be unable to recreate the dynamics. Therefore, the more steps one has to take, the worse. With large step sizes, one can find a model that connects states which lie far apart from each other. This will itself be unable to make good predictions for longer time spans but is suitable for few large steps.
%\begin{figure}[ht!]
%\centering
%\includegraphics[width=\textwidth]{Bilder/Lorenz96_errorPlot_overK.png}
%\caption{With increasing $K$, the prediction error decreases (except for from $K=5$ to $K=6$. The SINDy error is low for small time steps but becomes bigger for larger time steps.}
%\label{fig:Lorenz96_errorPlot_overK}
%\end{figure}



\begin{comment}
\begin{remark}
If $\clus > \memory+1$, then one might observe that in \eref{eq:SPA1} it would be enough to place $\dimD+1$ reference points so that all data are contained in $conv(\Smatrix)$ and the remaining ones can be placed arbitrarily. As is explained in \cite{spa}, one can impose a regularization on the mutual distances between the $\Spoint_i$ in the 2-norm by adding
\begin{equation*}
    \sum\limits_{k=1}^\clus \sum\limits_{j=k+1}^\clus \Vert \Spoint_k - \Spoint_j\Vert_2
\end{equation*}
to the $\data - \Smatrix\Gamma$ in \eqref{eq:SPA1}. This ensures that reference points should be evenly spaced
\end{remark}
\end{comment}


\iffalse
\subsection*{Linear approximations of the dynamics are insufficient to predict long-term behaviour}
\label{sec:SPAfixedpoints}
With \eqref{eq:SPA2}, we find a matrix $\Lambda$ that propagates projection coordinates linearly over time. The linearity plus the fact, that $\Lambda$ is a column-stochastic matrix, give severe restrictions on the capacities regarding long-term behaviour of the method: By the Perron-Frobenius Theorem, a full-rank column-stochastic matrix must have eigenvalues $\lambda_i$ with $|\lambda_i| \leq 1$ and at least (and generally exactly) one real eigenvalue $\lambda_1 = 1$. As a consequence, we can write subsequent application of $\Lambda$ using its eigenvectors: Let $u_1,\dots,u_\clus$ be the right eigenvectors of $\Lambda$. Then they form a basis of $\R^\clus$. Let $\gamma_t$ have a representation with respect to these eigenvectors given by
\begin{equation*}
    \gamma_t = \sum\limits_{k=1}^\clus a_k u_k
\end{equation*}
where the $a_k$ are real coefficients.
Then
\begin{equation*}
    \Lambda^i \gamma_t = \sum\limits_{k=1}^\clus a_k \Lambda^i u_k = \sum\limits_{k=1}^\clus a_k \lambda_k^i u_k.
\end{equation*}
All $\lambda_k$ where $|\lambda_j| < 1$ will vanish with increasing $i$, so that the sum converges to
\begin{equation*}
    \gamma^{\star} = a_1 u_1
\end{equation*}
(or, more generally, to $\sum\limits_{k:\lambda_k = 1} a_k u_k$).
Thus, in the long-term, a trajectory of projected coordinates created using the linear model must converge to a fixed point. Hence, also in the full state space a long-term prediction must converge to the fixed point $\datapoint^{\star} = \Smatrix \gamma^{\star}$. For systems that remain on attractors of higher dimension, e.g., that stay on a cycle infinitely long, such a linear model is therefore unable to capture the long-term behaviour.

Regarding the stability of the fixed point, we can make the following observation: By definition, a fixed point $\gamma^{\star}$ fulfills
\begin{equation*}
    \Lambda \gamma^{\star} = \gamma^{\star}.
\end{equation*}
The derivative of the function $h(\gamma) = \Lambda \gamma$ is $\Lambda$ itself, since it is a linear mapping. Since $\Lambda$ is a stochastic matrix and the dominant eigenvalue is equal to $1$, this means that $\gamma^{\star}$ is a Lyapunov stable fixed point. As such, all realisations that start close to $\gamma^{\star}$ remain close to it.

\fi
